Learning with Less: Knowledge Distillation from Large Language Models via Unlabeled Data

In real-world NLP applications, Large Language Models (LLMs) offer promising solutions due to their extensive training on vast datasets. However, the large size and high computation demands of LLMs limit their practicality in many applications, especially when further fine-tuning is required. To address these limitations, smaller models are typically preferred for deployment. However, their training is hindered by the scarcity of labeled data. In contrast, unlabeled data is often readily which can be leveraged by using LLMs to generate pseudo-labels for training smaller models. This enables the smaller models (student) to acquire knowledge from LLMs(teacher) while reducing computational costs. This process introduces challenges, such as potential noisy pseudo-labels. Selecting high-quality and informative data is therefore critical to enhance model performance while improving the efficiency of data utilization. To address this, we propose LLKD that enables Learning with Less computational resources and less data for Knowledge Distillation from LLMs. LLKD is an adaptive sample selection method that incorporates signals from both the teacher and student. Specifically, it prioritizes samples where the teacher demonstrates high confidence in its labeling, indicating reliable labels, and where the student exhibits a high information need, identifying challenging samples that require further learning. Our comprehensive experiments show that LLKD achieves superior performance across various datasets with higher data efficiency.

==> sections/preliminary.tex <==

\begin{figure*}[t]
\begin{center}
 \centering
\includegraphics[width=0.95\linewidth]{figures/framework.pdf} 
\caption{An illustration of the knowledge distillation framework.  } \sn{Can we improve this figure? Just visually looks a bit like a draft figure}
\label{fig:framework}
\end{center}

\end{figure*}

\section{Preliminary}
Given the unlabeled dataset $\mathcal{X} =  \{x_1, x_2, ..., x_N\}$ where $ x_i \in \mathcal{X}$ is the input text, we do not have labels for the samples in $\mathcal{X}$. However, we are provided with a label set  $\mathcal{Y} = \{y_1, y_2, ..., y_K\}$  
 consisting of $K$ possible labels, where each $y_i \in \mathcal{Y}$ is the $i$-th label words. For model training, we use $\mathcal{X}$ as the training set.
  To evaluate the performance, we have the validation and test set $\mathcal{X}_{dev}= \{ (x_j, y_j)\}_j^{M_1}$, $\mathcal{X}_{test}= \{ (x_j, y_j)\}_j^{M_2}$, where both sets contain the ground truth labels.  The validation set is used to select the model.

\sw{the following is more like an overview of our framework, instead of preliminary. Consider merging it with the first paragraph of Section 4?}We leverage the unlabeled data to train the smaller model using pseudo-labels generated by the teacher LLM. Let $G_t$ denote the teacher LLM (e.g., LLaMA~\cite{touvron2023llama}), and $G_s$ represent the student language model (e.g., RoBERTa~\cite{liu2019roberta}). The framework of the proposed method is illustrated in \figurename~\ref{fig:framework}. The teacher LLM remains fixed and is only used for inference.
A key step of this framework is selecting samples with both high pseudo-label quality and high informativeness for the student. To achieve this, we use the teacher's confidence to indicate pseudo-label quality, where higher teacher confidence indicates more reliable labels. Additionally, we use the student's uncertainty to identify hard samples, where greater uncertainty indicates challenging knowledge that require further training.
We integrate signals from both the teacher and student models to select samples with high pseudo-label quality that are also informative for the student. These carefully selected samples are then used to train the student model, significantly reducing the number of samples required, thereby improving the data efficiency while striving to optimize model performance. 
